Determining stellar accretion rates from $Pa_{\alpha}$ and $Br_{\beta}$ emission lines with JWST NIRSpec

In this letter we present the first systematic spectroscopic measurements of the Near-InfraRed (NIR) hydrogen recombination lines Paschen alpha ($Pa_{\alpha}$ $\lambda = 1.875 \mu m$) and Brackett beta ($Br_{\beta}$ $\lambda = 2.626 \mu m$), produced by pre-main-sequence (PMS) stars. These stars, consisting of T Tauri and Herbig AeBe stars are located in the massive Galactic star-formation region NGC 3603. The measurements were obtained from JWST NIRSpec, using multi-object spectroscopy (MOS) mode. Utilising existing empirical relations between $L_{acc}$ and $L_{Br_{\gamma}}$, we have used our new measurements to formulate, for the first time, an empirical relationship between the accretion luminosity $L_{acc}$ of the stars, and the line luminosities $L_{line}$ of both $Pa_{\alpha}$ and $Br_{\beta}$. These relationships are: $\log_{10}( \frac{L_{acc}}{L_{\odot}}) = 1.42 (\pm 0.18) \times \log_{10}( \frac{L_{Pa_{\alpha}}}{L_{\odot}}) + 3.33 (\pm 0.42)$ and $\log_{10}( \frac{L_{acc}}{L_{\odot}}) = 1.47 (\pm 0.18) \times \log_{10}( \frac{L_{Br_{\beta}}}{L_{\odot}}) + 4.60 (\pm 0.57)$. These new relationships are key for roughly estimating the accretion rates for large samples of PMS stars with JWST.

==> name.tex <==
% \begin{table*}
% \small
%     \centering
%     \begin{tabular}{ccccccccccc}
%          \hline
%          ID&  RA&  DEC&  $T_{eff}$ (K)&  Group &$M_*$ ($M_{\odot}$)&  EW $Pa_{\alpha}$ ($\AA$)&  EW $Br_{\gamma}$ ($\AA$)&  EW $Br_{\beta}$ ($\AA$)&  $L_{acc}$ $(L_{\odot})$& \\
%          \hline
%          \hline
%          727& 168.8096466& -61.263581& 3800 $\pm 150$&  TT&0.5 $\pm 0.06$& -23.1 $\pm 2.2$& -0.8 $\pm 0.2$& -9.7 $\pm 1.9$& -1.42 $\pm 0.75$\\ 
%          654&  168.7541941&  -61.2514463&  4600 $\pm 150$&   TT&0.75 $\pm 0.07$&  -3.6 $\pm 0.4$&  -0.4 $\pm 0.1$&  -3.8 $\pm 0.7$&  -1.419& \\ 
%          4595&  168.8129136&  -61.2625111&  3600 $\pm 150$&   TT&0.47 $\pm 0.05$&  -22.2 $\pm 2$&  -2.4 $\pm 0.7$&  -26 $\pm 4.7$&  -1.401& \\ 
%          996&  168.7973597&  -61.2640824&  5200 $\pm 150$&   TT&0.97 $\pm 0.08$&  -8.9 $\pm 0.7$&  -0.5 $\pm 0.2$&  -2.9 $\pm 0.5$&  -1.113& \\ 
%          1497&  168.7688519&  -61.25128&  6000 $\pm 100$&   TT&1.3 $\pm 0.04$&  -24.2 $\pm 2$&  -2.9 $\pm 0.5$&  -17.1 $\pm 2.9$&  -1.077& \\ 
%          1457&  168.7310205&  -61.2672106&  5400 $\pm 100$&   TT&1.05 $\pm 0.04$&  -45.5 $\pm 3.8$&  -10.7 $\pm 1.3$&  -61 $\pm 10.5$&  -0.749& \\ 
%          1038&  168.7957658&  -61.2643274&  5400 $\pm 150$&   TT&1.05 $\pm 0.08$&  -54.2 $\pm 4.6$&  -3.6 $\pm 0.5$&  -12.2 $\pm 2$&  -0.747& \\ 
%          1339&  168.8197744&  -61.2630422&  4400 $\pm 150$&   TT&0.7 $\pm 0.06$&  -12 $\pm 1$&  -5.7 $\pm 0.7$&  -45 $\pm 7.8$&  -0.733& \\ 
%          858&  168.7365507&  -61.2702015&  9600 $\pm 200$&   HBe$^{*}$&3.3 $\pm 0.14$&  -82.6 $\pm 6.9$&  -7.6 $\pm 0.8$&  -33.5 $\pm 5.9$&  -0.667& \\ 
%          1813&  168.8037358&  -61.246069&  5600 $\pm 150$&   TT&1.1 $\pm 0.08$&  -48 $\pm 4.1$&  -5.6 $\pm 0.7$&  -38 $\pm 6.7$&  -0.654& \\ 
%          1442&  168.8120917&  -61.2671703&  4200 $\pm 150$&   TT&0.65 $\pm 0.06$&  -11 $\pm 0.9$&  -1 $\pm 0.2$&  -2.4 $\pm 0.4$&  -0.648& \\ 
%          1997&  168.8052566&  -61.2510052&  4400 $\pm 200$&   TT&0.7 $\pm 0.06$&  -14.8 $\pm 1.3$&  -1.3 $\pm 0.2$&  -3.2 $\pm 0.6$&  -0.61& \\ 
%          1717&  168.8138352&  -61.2507679&  5800 $\pm 200$&   TT&1.2 $\pm 0.08$&  -24.6 $\pm 2.1$&  -3.4 $\pm 0.6$&  -6.7 $\pm 1.2$&  -0.605& \\ 
%          4649&  168.7420813&  -61.2585345&  3600 $\pm 150$&   TT&0.47 $\pm 0.05$&  -128.7 $\pm 11.7$&  -10.6 $\pm 1.8$&  -59.3 $\pm 10.6$&  -0.528& \\ 
%          1271&  168.7330151&  -61.2635352&  4600 $\pm 200$&   TT&0.75 $\pm 0.07$&  -70.6 $\pm 6$&  -9 $\pm 1.1$&  -17.5 $\pm 3.1$&  -0.468& \\ 
%          2326&  168.7438995&  -61.2588048&  3800 $\pm 150$&   TT&0.5 $\pm 0.06$&  -114.3 $\pm 10.1$&  -25.7 $\pm 4.4$&  -86.3 $\pm 16.3$&  -0.413& \\ 
%          1134&  168.7353906&  -61.2705277&  5600 $\pm 150$&   TT&1.13 $\pm 0.08$&  -125.1 $\pm 10.5$&  -10.1 $\pm 1.2$&  -45.4 $\pm 8.1$&  -0.371& \\ 
%          2673&  168.7975961&  -61.2649162&  4400 $\pm 100$&   TT&0.7 $\pm 0.03$&  -34.2 $\pm 3$&  -3.5 $\pm 0.5$&  -7.3 $\pm 1.4$&  -0.361& \\ 
%          1854&  168.7292443&  -61.2600537&  4200 $\pm 150$&   TT&0.75 $\pm 0.07$&  -225.1 $\pm 19.7$&  -22.8 $\pm 2.9$&  -127.9 $\pm 22.3$&  -0.356& \\ 
%          2492&  168.7427501&  -61.2714228&  5000 $\pm 100$&   TT&0.9 $\pm 0.04$&  -245 $\pm 21.8$&  -57.6 $\pm 7$&  -79.2 $\pm 14.7$&  -0.27& \\ 
%          977&  168.8092518&  -61.2623119&  5000 $\pm 150$&   TT&0.9 $\pm 0.07$&  -19.1 $\pm 1.6$&  -2 $\pm 0.3$&  -5.8 $\pm 1.1$&  -0.028& \\ 
%          354&  168.7704651&  -61.2626355&  10600 $\pm 2000$&   HBe&$4.02^{+1.7}_{-1.2}$&  -22.5 $\pm 2.1$&  -5 $\pm 1.3$&  -5.6 $\pm 1.3$&  0.068& \\ 
%          853&  168.7643462&  -61.2488318&  5400 $\pm 100$&   TT&1.05 $\pm 0.04$&  -18.2 $\pm 1.5$&  -2.1 $\pm 0.3$&  -5.9 $\pm 0.9$&  0.154& \\ 
%          2166&  168.7944201&  -61.2661562&  5000 $\pm 150$&   TT&0.9 $\pm 0.07$&  -69.1 $\pm 6.2$&  -6.5 $\pm 0.8$&  -15.3 $\pm 2.6$&  0.273& \\ 
%          152&  168.7817328&  -61.2648809&  9400 $\pm 1800$&   HBe&$4.33^{+1.8}_{-1.3}$&  -14.9 $\pm 1.2$&  -1.5 $\pm 0.2$&  -2.2 $\pm 0.4$&  0.415& \\ 
%          1350&  168.8031179&  -61.2483281&  -&  -&-&  -53.6 $\pm 4.4$&  -8.2 $\pm 1$&  -11.1 $\pm 2$&  0.661& \\ 
%          1354&  168.7519521&  -61.2645637&  6600 $\pm 1400$&   HAe&$2.18^{+ 0.90}_{-0.64}$&  -20.8 $\pm 1.7$&  -3.5 $\pm 0.4$&  -5 $\pm 0.8$&  0.898& \\ 
%          823&  168.7623889&  -61.2710101&  7200 $\pm 1400$&   HAe&$3.13^{+ 1.3}_{-0.92}$&  -33.8 $\pm 2.9$&  -6 $\pm 0.7$&  -9 $\pm 1.5$&  1.785& \\ 
%          238&  168.8151779&  -61.2550836&  7000 $\pm 1800$&   HBe&$5.47^{+ 2.3}_{-1.6}$&  -76 $\pm 6.3$&  -13.5 $\pm 2.1$&  -23.6 $\pm 4.2$&  2.064& \\ 
%          185&  168.7627924&  -61.2625057&  8200 $\pm 1800$&   HBe&$5.06^{+ 2.1}_{-1.5}$&  -82.2 $\pm 6.8$&  -9.4 $\pm 1.1$&  -14.1 $\pm 2.3$&  2.131& \\ 
%          35&  168.8077768&  -61.2661962&  29000 $\pm 1800$&   HBe&$5.56^{+ 2.3}_{-1.6}$&  -46.6 $\pm 4$&  -15.8 $\pm 1.9$&  -40.1 $\pm 6.9$&  2.482& \\ 
%          469&  168.7941589&  -61.2779717&  8600 $\pm 1800$&   HBe&$5.16^{+ 2.1}_{-1.5}$&  -216.9 $\pm 45.1$&  -16.2 $\pm 2$&  -17.2 $\pm 3.1$&  2.518& \\ 
%          251& 168.7684956& -61.2531283& 6400 $\pm 1800$&  HBe&$3.74^{+ 1.5}_{-1.1}$& -124.9 $\pm 10.6$& -13.7 $\pm 1.6$& -17.6 $\pm 3.1$& 2.751&\\ 
%     \end{tabular}
%     \caption{\textbf{\small{The physical properties of the PMS stars considered in this analysis, as well as the EWs of the three recombination lines. The sources have been ordered in terms of increasing accretion luminosity. The Group column indicates whether the sources are classified as T Tauri, Herbig Ae or Herbig Be stars. For the T Tauri stars, the temperatures, masses and associated uncertainties come directly from the Phoenix stellar models based on the 5 best fitting model spectra. For the Herbig AeBe stars, the temperatures and masses come from the photometry of (B10). The uncertainty in mass for each source has been calculated based on $M_{*} \divideontimes \sqrt{2}$. The uncertainty in temperature for the Herbig AeBe stars has been determined from the Phoenix models, such that the range of temperature reproduces the upper and lower mass limit for each source.\\ 
%     \textbf{Note.} Source 858 has been marked with $*$ to denote that it has been classified as a Herbig Be directly via spectroscopy. As such its temperature, mass and uncertainties have been determined in the same way as the T Tauri stars. Source 1350 could not be classified by spectroscopic or photometric means.}}}
%     \label{tab:all_sources}
% \end{table*}
